GuidedRec: Guiding Ill-Posed Unsupervised Volumetric Recovery

We introduce a novel unsupervised approach to reconstructing a 3D volume from only two planar projections that exploits a previous\-ly-captured 3D volume of the patient. Such volume is readily available in many important medical procedures and previous methods already used such a volume. Earlier methods that work by deforming this volume to match the projections typically fail when the number of projections is very low as the alignment becomes underconstrained. We show how to use a generative model of the volume structures to constrain the deformation and obtain a correct estimate. Moreover, our method is not bounded to a specific sensor calibration and can be applied to new calibrations without retraining. We evaluate our approach on a challenging dataset and show it outperforms state-of-the-art methods. As a result, our method could be used in treatment scenarios such as surgery and radiotherapy while drastically reducing patient radiation exposure.

==> 4t_metrics.tex <==
\begin{table}
\centering
\caption{\textbf{Metrics on volumes  from two projections by previous methods and our approach.}
Standard deviations are provided in parentheses. (w/) and (w/o) stand for the use or not of the pre-captured volume respectively.
\alexandrermk{seems X2Vision is working well for registration as well, may be coarser with less details than 2d3dNR but more matching of big structures - there is no issue of downsampling upsamling also for it as doesnt take the ct}
}
\label{tab:metrics}
\addtolength{\tabcolsep}{+1pt}
%
\scalebox{0.9}{
\begin{tabular}{@{}lcc@{}}
\toprule
\multicolumn{1}{c}{Method} & PSNR~(dB) $\uparrow$ &  SSIM $\uparrow$ \\ 
\midrule
Backprojection & $10.29~(\pm 0.5)$ & $0.23~(\pm 0.01)$ \\[1.1mm]
NeRP (w/o)~\cite{shen2022nerp}  & $19.81~(\pm 1.7)$ & $0.21~(\pm 0.03)$ \\[1.mm]
NeRP (w/)~\cite{shen2022nerp} & $25.32~(\pm 1.6)$ & $0.34~(\pm 0.02)$ \\[1.mm]
X2Vision~\cite{x2vision} & $27.80~(\pm 1.4)$ & $0.89~(\pm 0.03)$ \\[1.mm]
2D3DNR~\cite{dong20232d} & $29.07~(\pm 1.6)$ & $0.92~(\pm 0.02)$ \\
\midrule
Ours & $\mathbf{33.23~(\pm 0.62)}$ & $\mathbf{0.96~(\pm 0.01)}$ \\

\bottomrule
\bottomrule

\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Dice $\uparrow$} \\
\cline{2-3} %\cline{5-6}
% \midrule
\multicolumn{1}{c}{} & Mouth & Larynx\\ 
\midrule
2D3DNR~\cite{dong20232d} & $0.91~(\pm 0.03)$ & $0.80~(\pm0.07)$ \\[1.mm]
Ours & $\mathbf{0.95~(\pm 0.01)}$ & $\mathbf{0.91~(\pm0.02)}$ \\

\bottomrule
\bottomrule
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Rigid Registration Error (6 DoF)} \\
\cline{2-3} %\cline{5-6}
% \midrule
\multicolumn{1}{c}{} & Rotation(°) $\downarrow$ & Translation(mm) $\downarrow$\\ 
\midrule

2D3DNR~\cite{dong20232d} & $0.52~(\pm 0.29)$ & $0.88~(\pm0.45)$ \\[1.mm]
X2Vision~\cite{x2vision} & $0.45~(\pm 0.31)$ & $0.50~(\pm0.26)$ \\[1.mm]
Ours & $\mathbf{0.16~(\pm 0.15)}$ & $\mathbf{0.20~(\pm0.07)}$ \\

\bottomrule

\end{tabular}
}
\end{table}
